HATS-1b: The First Transiting Planet Discovered by the HATSouth Survey

We report the discovery of HATS-1b, a transiting extrasolar planet orbiting the moderately bright V=12.05 G dwarf star GSC 6652-00186, and the first planet discovered by HATSouth, a global network of autonomous wide-field telescopes. HATS-1b has a period P~3.4465 d, mass Mp~1.86MJ, and radius Rp~1.30RJ. The host star has a mass of 0.99Msun, and radius of 1.04Rsun. The discovery light curve of HATS-1b has near continuous coverage over several multi-day periods, demonstrating the power of using a global network of telescopes to discover transiting planets.

==> HATS563-036.tex <==
\newcommand{\hatcurhtr}{HATS563-036}                                   % Original HTR name of target
\newcommand{\hatcurfield}{563}                                         % Original HTR field
\newcommand{\hatcurCCra}{\ensuremath{11^{\mathrm h}42^{\mathrm m}06.12{\mathrm s}}}                                  % Right Ascension
\newcommand{\hatcurCCdec}{\ensuremath{-23{\arcdeg}21{\arcmin}17.4{\arcsec}}}                                 % Declination
\newcommand{\hatcurCCmag}{12.053}                                      % apparent V-band magnitude
\newcommand{\hatcurCCtwomass}{2MASS~11420608-2321174}                  % 2MASS identifier
\newcommand{\hatcurCCgsc}{GSC~6652-00186}                              % GSC(1.2) identifier
\newcommand{\hatcurCCapassmVshort}{\ensuremath{12.05}}                % V-band magnitude
\newcommand{\hatcurCCapassmV}{\ensuremath{12.053\pm0.017}}             % APASS V-band magnitude
\newcommand{\hatcurCCapassmB}{\ensuremath{12.740\pm0.066}}              % APASS B-band magnitude
\newcommand{\hatcurCCapassmg}{\ensuremath{12.356\pm0.052}}             % APASS g-band magnitude
\newcommand{\hatcurCCapassmr}{\ensuremath{11.866\pm0.045}}             % APASS r-band magnitude
\newcommand{\hatcurCCapassmi}{\ensuremath{11.748\pm0.042}}             % APASS i-band magnitude
%% --------------------------------------------------------------------
\newcommand{\hatcurCCtwomassJmag}{\ensuremath{10.924\pm0.024}}         % 2MASS ORIG MAG
\newcommand{\hatcurCCtwomassHmag}{\ensuremath{10.634\pm0.022}}         % 2MASS ORIG MAG
\newcommand{\hatcurCCtwomassKmag}{\ensuremath{10.580\pm0.023}}         % 2MASS ORIG MAG
\newcommand{\hatcurCCcitJmag}{\ensuremath{10.942\pm0.024}}             % 2MASS CIT MAG
\newcommand{\hatcurCCcitHmag}{\ensuremath{10.629\pm0.022}}             % 2MASS CIT MAG
\newcommand{\hatcurCCcitKmag}{\ensuremath{10.604\pm0.023}}             % 2MASS CIT MAG
\newcommand{\hatcurCCbbJmag}{\ensuremath{10.989\pm0.026}}              % 2MASS BB MAG
\newcommand{\hatcurCCbbHmag}{\ensuremath{10.650\pm0.023}}              % 2MASS BB MAG
\newcommand{\hatcurCCbbKmag}{\ensuremath{10.624\pm0.023}}              % 2MASS BB MAG
\newcommand{\hatcurCCesoJmag}{\ensuremath{10.991\pm0.027}}             % 2MASS ESO MAG
\newcommand{\hatcurCCesoHmag}{\ensuremath{10.644\pm0.026}}             % 2MASS ESO MAG
\newcommand{\hatcurCCesoKmag}{\ensuremath{10.623\pm0.024}}             % 2MASS ESO MAG
\newcommand{\hatcurCCesoJHmag}{\ensuremath{0.346\pm0.035}}             % 2MASS ESO JH COLOR
\newcommand{\hatcurCCesoJKmag}{\ensuremath{0.369\pm0.036}}             % 2MASS ESO JK COLOR
\newcommand{\hatcurCCesoHKmag}{\ensuremath{0.022\pm0.035}}             % 2MASS ESO HK COLOR
%% --------------------------------------------------------------------
\newcommand{\hatcurLCdip}{\ensuremath{13.8}}                           % BLS detected dip (mmag)
\newcommand{\hatcurLCrprstar}{\ensuremath{0.1288\pm0.0020}}            % Rp/R*
\newcommand{\hatcurLCbsq}{\ensuremath{0.400_{-0.028}^{+0.026}}}        % impact parameter square
\newcommand{\hatcurLCimp}{\ensuremath{0.633_{-0.023}^{+0.020}}}        % impact parameter
\newcommand{\hatcurLCzeta}{\ensuremath{23.98\pm0.16}}                  % zeta/R*
\newcommand{\hatcurLCdur}{\ensuremath{0.1007\pm0.0012}}                % transit duration (days)
\newcommand{\hatcurLCdurshort}{\ensuremath{0.1007}}                    % transit duration (days)
\newcommand{\hatcurLCdurhr}{\ensuremath{2.416\pm0.028}}                % transit duration (hours)
\newcommand{\hatcurLCdurhrshort}{\ensuremath{2.416}}                   % transit duration (hours)
\newcommand{\hatcurLCq}{\ensuremath{0.0292\pm0.0003}}                  % fractional transit duration (days)
\newcommand{\hatcurLCqshort}{\ensuremath{0.029}}                       % fractional transit duration (days)
\newcommand{\hatcurLCingdur}{\ensuremath{0.0181\pm0.0011}}             % ingress/egress duration (days)
\newcommand{\hatcurLCP}{\ensuremath{3.446459\pm0.000004}}              % period (days)
\newcommand{\hatcurLCPprec}{\ensuremath{3.4464588}}                    % period (days)
\newcommand{\hatcurLCPshort}{\ensuremath{3.4465}}                      % period (days)
\newcommand{\hatcurLCT}{\ensuremath{2455241.28722\pm0.00071}}          % epoch (BJD)
\newcommand{\hatcurLCTA}{\ensuremath{2455217.16201\pm0.00073}}         % TA (BJD)
\newcommand{\hatcurLCTB}{\ensuremath{2455747.91667\pm0.00030}}         % TB (BJD)
\newcommand{\hatcurLChatnetmA}{\ensuremath{11.9826\pm0.0001}}          % HATNet OOT level
\newcommand{\hatcurLCiblendA}{\ensuremath{0.79\pm0.03}}                % HATNet iblend factor
\newcommand{\hatcurLChatnetmB}{\ensuremath{10.3359\pm0.0005}}          % HATNet OOT level
\newcommand{\hatcurLCiblendB}{\ensuremath{-0.10\pm0.00}}               % HATNet iblend factor
%% --------------------------------------------------------------------
\newcommand{\hatcurSPCiteff}{\ensuremath{5870\pm100}}                  % Ini SPC, stellar effective temperature
\newcommand{\hatcurSPCizfeh}{\ensuremath{-0.06\pm0.12}}                % Ini SPC, stellar metallicity
\newcommand{\hatcurSPCizfehshort}{\ensuremath{-0.06}}                  % Ini SPC, stellar metallicity
\newcommand{\hatcurSPCilogg}{\ensuremath{4.52\pm0.15}}                 % Ini SPC, stellar surface gravity
\newcommand{\hatcurSPCivsin}{\ensuremath{2.52\pm0.5}}                  % Ini SPC, stellar rotational velocity
\newcommand{\hatcurSPCivmac}{\ensuremath{NULL}}                        % Ini SPC, stellar macroturbulence
\newcommand{\hatcurSPCivmic}{\ensuremath{NULL}}                        % Ini SPC, stellar microturbulence
\newcommand{\hatcurSPCiiteff}{\ensuremath{5814\pm100}}                 % Final SPC, stellar effective temperature
\newcommand{\hatcurSPCiizfeh}{\ensuremath{-0.1\pm0.1}}                 % Final SPC, stellar metallicity
\newcommand{\hatcurSPCiizfehshort}{\ensuremath{-0.1}}                  % Final SPC, stellar metallicity
\newcommand{\hatcurSPCiilogg}{\ensuremath{4.40\pm0.08}}                % Final SPC, stellar surface gravity
\newcommand{\hatcurSPCiivsin}{\ensuremath{2.60\pm0.5}}                 % Final SPC, stellar rotational velocity
\newcommand{\hatcurSPCiivmac}{\ensuremath{NULL}}                       % Final SPC, stellar macroturbulence
\newcommand{\hatcurSPCiivmic}{\ensuremath{NULL}}                       % Final SPC, stellar microturbulence
%% --------------------------------------------------------------------
\newcommand{\hatcurDSteff}{\ensuremath{NULL\pmNULL}}                   % DS stellar effective temperature
\newcommand{\hatcurDSzfeh}{\ensuremath{NULL\pmNULL}}                   % DS stellar metallicity
\newcommand{\hatcurDSlogg}{\ensuremath{NULL\pmNULL}}                   % DS stellar surface gravity
\newcommand{\hatcurDSvsini}{\ensuremath{NULL\pmNULL}}                  % DS stellar rotational velocity
\newcommand{\hatcurDSgamma}{\ensuremath{NULL\pmNULL}}                  % DS absolute gamma velocity
\newcommand{\hatcurDSnumspec}{\ensuremath{0}}                          % DS number of spectra
\newcommand{\hatcurDSspan}{\ensuremath{0}}                             % DS stellar surface gravity
\newcommand{\hatcurDSrvrms}{\ensuremath{0.00}}                         % DS rms of RV values [km/s]
%% --------------------------------------------------------------------
\newcommand{\hatcurTRESteff}{\ensuremath{NULL\pmNULL}}                 % TRES stellar effective temperature
\newcommand{\hatcurTRESzfeh}{\ensuremath{NULL\pmNULL}}                 % TRES stellar metallicity
\newcommand{\hatcurTRESlogg}{\ensuremath{NULL\pmNULL}}                 % TRES stellar surface gravity
\newcommand{\hatcurTRESvsini}{\ensuremath{NULL\pmNULL}}                % TRES stellar rotational velocity
\newcommand{\hatcurTRESgamma}{\ensuremath{NULL\pmNULL}}                % TRES absolute gamma velocity
\newcommand{\hatcurTRESnumspec}{\ensuremath{0}}                        % TRES number of spectra
\newcommand{\hatcurTRESspan}{\ensuremath{0}}                           % TRES stellar surface gravity
\newcommand{\hatcurTRESrvrms}{\ensuremath{0.00}}                       % TRES rms of RV values [km/s]
%% --------------------------------------------------------------------
\newcommand{\hatcurFIESteff}{\ensuremath{NULL\pmNULL}}                 % FIES stellar effective temperature
\newcommand{\hatcurFIESzfeh}{\ensuremath{NULL\pmNULL}}                 % FIES stellar metallicity
\newcommand{\hatcurFIESlogg}{\ensuremath{NULL\pmNULL}}                 % FIES stellar surface gravity
\newcommand{\hatcurFIESvsini}{\ensuremath{NULL\pmNULL}}                % FIES stellar rotational velocity
\newcommand{\hatcurFIESgamma}{\ensuremath{NULL\pmNULL}}                % FIES absolute gamma velocity
\newcommand{\hatcurFIESnumspec}{\ensuremath{0}}                        % FIES number of spectra
\newcommand{\hatcurFIESspan}{\ensuremath{0}}                           % FIES stellar surface gravity
\newcommand{\hatcurFIESrvrms}{\ensuremath{0.00}}                       % FIES rms of RV values [km/s]
%% --------------------------------------------------------------------
\newcommand{\hatcurLBiz}{\ensuremath{0.1986}}                          % Limb darkening parameters, Gamma1, z-band
\newcommand{\hatcurLBiiz}{\ensuremath{0.3280}}                         % Limb darkening parameters, Gamma2, z-band
\newcommand{\hatcurLBii}{\ensuremath{0.2560}}                          % Limb darkening parameters, Gamma1, i-band
\newcommand{\hatcurLBiii}{\ensuremath{0.3331}}                         % Limb darkening parameters, Gamma2, i-band
\newcommand{\hatcurLBiI}{\ensuremath{0.2366}}                          % Limb darkening parameters, Gamma1, I-band
\newcommand{\hatcurLBiiI}{\ensuremath{0.3319}}                         % Limb darkening parameters, Gamma2, I-band
\newcommand{\hatcurLBig}{\ensuremath{0.5230}}                          % Limb darkening parameters, Gamma1, g-band
\newcommand{\hatcurLBiig}{\ensuremath{0.2574}}                         % Limb darkening parameters, Gamma2, g-band
\newcommand{\hatcurLBir}{\ensuremath{0.3387}}                          % Limb darkening parameters, Gamma1, r-band
\newcommand{\hatcurLBiir}{\ensuremath{0.3343}}                         % Limb darkening parameters, Gamma2, r-band
\newcommand{\hatcurLBiR}{\ensuremath{0.3158}}                          % Limb darkening parameters, Gamma1, R-band
\newcommand{\hatcurLBiiR}{\ensuremath{0.3349}}                         % Limb darkening parameters, Gamma2, R-band
\newcommand{\hatcurLBikep}{\ensuremath{}}                      % darkening parameters, Gamma1, Kep-band
\newcommand{\hatcurLBiikep}{\ensuremath{}}                     % darkening parameters, Gamma2, Kep-band
%% --------------------------------------------------------------------
\newcommand{\hatcurISOm}{\ensuremath{0.99\pm0.05}}                     % stellar mass
\newcommand{\hatcurISOmshort}{\ensuremath{0.99}}                       % stellar mass
\newcommand{\hatcurISOmlong}{\ensuremath{0.986\pm0.054}}               % stellar mass
\newcommand{\hatcurISOr}{\ensuremath{1.04_{-0.08}^{+0.13}}}            % stellar radius
\newcommand{\hatcurISOrshort}{\ensuremath{1.04}}                       % stellar radius
\newcommand{\hatcurISOrlong}{\ensuremath{1.038_{-0.075}^{+0.128}}}     % stellar radius
\newcommand{\hatcurISOrho}{\ensuremath{1.24\pm0.32}}                   % stellar density (cgs)
\newcommand{\hatcurISOlogg}{\ensuremath{4.40\pm0.08}}                  % stellar surface gravity from isochrones
\newcommand{\hatcurISOlum}{\ensuremath{1.10_{-0.18}^{+0.33}}}          % stellar luminosity
\newcommand{\hatcurISOlumshort}{\ensuremath{1.10}}                     % stellar luminosity
\newcommand{\hatcurISOmv}{\ensuremath{4.73\pm0.24}}                    % stellar absolute magnitude
\newcommand{\hatcurISOvi}{\ensuremath{0.684\pm0.029}}                  % stellar V-I index
\newcommand{\hatcurISOage}{\ensuremath{6.0\pm2.8}}                     % stellar age
\newcommand{\hatcurISOsigma}{\ensuremath{0.00230\pm0.00042}}           % system mass-correction sigma parameter
\newcommand{\hatcurISOMJ}{\ensuremath{3.60\pm0.22}}                    % stellar absolute J magnitude
\newcommand{\hatcurISOMH}{\ensuremath{3.27\pm0.22}}                    % stellar absolute H magnitude
\newcommand{\hatcurISOMK}{\ensuremath{3.21\pm0.22}}                    % stellar absolute K magnitude
\newcommand{\hatcurISOJK}{\ensuremath{0.39\pm0.02}}                    % J-K color index from isochrones.
\newcommand{\hatcurISOspec}{G}                                         % stellar spectral type
%% --------------------------------------------------------------------
\newcommand{\hatcurRVK}{\ensuremath{254.1\pm33.1}}                     % RV semi-amplitude [m/s]
\newcommand{\hatcurRVk}{\ensuremath{-0.064_{-0.064}^{+0.041}}}         % e*cos(omega)
\newcommand{\hatcurRVh}{\ensuremath{0.097_{-0.073}^{+0.102}}}          % e*sin(omega)
\newcommand{\hatcurRVtrone}{\ensuremath{0.0000\pm0.0000}}              % RV linear trend tr1 factor
\newcommand{\hatcurRVtrtwo}{\ensuremath{0.0000\pm0.0000}}              % RV linear trend tr2 factor
\newcommand{\hatcurRVgammaA}{\ensuremath{-138.1\pm22.3}}               % RV gamma velocity, relative scale
\newcommand{\hatcurRVjitterA}{\ensuremath{0.0}}                        % RV jitter (m/s)
\newcommand{\hatcurRVfitrmsA}{\ensuremath{19.6}}                       % RVfitrms
\newcommand{\hatcurRVgammaB}{\ensuremath{-81.7\pm22.6}}                % RV gamma velocity, relative scale
\newcommand{\hatcurRVjitterB}{\ensuremath{61.5}}                       % RV jitter (m/s)
\newcommand{\hatcurRVfitrmsB}{\ensuremath{84.9}}                       % RVfitrms
\newcommand{\hatcurRVgammaC}{\ensuremath{12.9\pm32.6}}                 % RV gamma velocity, relative scale
\newcommand{\hatcurRVjitterC}{\ensuremath{60.5}}                       % RV jitter (m/s)
\newcommand{\hatcurRVfitrmsC}{\ensuremath{65.1}}                       % RVfitrms
\newcommand{\hatcurRVeccen}{\ensuremath{0.120\pm0.092}}                % eccentricity
\newcommand{\hatcurRVomega}{\ensuremath{124\pm44}}                     % argument of pericenter
%% --------------------------------------------------------------------
\newcommand{\hatcurPPi}{\ensuremath{85.6_{-1.4}^{+0.6}}}               % orbital inclination
\newcommand{\hatcurPPg}{\ensuremath{26.8\pm4.4}}                       % planetary surface gravity (m/s^2)
\newcommand{\hatcurPPlogg}{\ensuremath{3.43\pm0.07}}                   % planetary surface gravity (log cgs)
\newcommand{\hatcurPPar}{\ensuremath{9.20\pm0.82}}                     % relative orbital radius (a/R*)
\newcommand{\hatcurPParel}{\ensuremath{0.0444\pm0.0008}}               % semimajor axis (AU)
\newcommand{\hatcurPPrho}{\ensuremath{1.03\pm0.25}}                    % planetary density (cgs)
\newcommand{\hatcurPPm}{\ensuremath{1.86_{-0.20}^{+0.26}}}             % planetary mass (M_jup)
\newcommand{\hatcurPPmshort}{\ensuremath{1.86}}                        % planetary mass (M_jup)
\newcommand{\hatcurPPmlong}{\ensuremath{1.855_{-0.196}^{+0.262}}}      % planetary mass (M_jup)
\newcommand{\hatcurPPme}{\ensuremath{589.7_{-62.3}^{+83.3}}}           % planetary mass (M_earth)
\newcommand{\hatcurPPmeshort}{\ensuremath{589.7}}                      % planetary mass (M_earth)
\newcommand{\hatcurPPmelong}{\ensuremath{589.68_{-62.33}^{+83.35}}}    % planetary mass (M_earth)
\newcommand{\hatcurPPr}{\ensuremath{1.30_{-0.10}^{+0.16}}}             % planetary radius (R_jup)
\newcommand{\hatcurPPrshort}{\ensuremath{1.30}}                        % planetary radius (R_jup)
\newcommand{\hatcurPPrlong}{\ensuremath{1.302_{-0.098}^{+0.162}}}      % planetary radius (R_jup)
\newcommand{\hatcurPPre}{\ensuremath{14.6_{-1.1}^{+1.8}}}              % planetary radius (R_earth)
\newcommand{\hatcurPPreshort}{\ensuremath{14.6}}                       % planetary radius (R_earth)
\newcommand{\hatcurPPrelong}{\ensuremath{14.59_{-1.10}^{+1.81}}}       % planetary radius (R_earth)
\newcommand{\hatcurPPmrcorr}{\ensuremath{0.53}}                        % mass/radius correlation
\newcommand{\hatcurPPteff}{\ensuremath{1359_{-59}^{+89}}}              % planetary temperature (K)
\newcommand{\hatcurPPtheta}{\ensuremath{0.127\pm0.014}}                % Safranov number
\newcommand{\hatcurPPfluxperi}{\ensuremath{9.86_{-2.41}^{+8.67}}}      % flux @ periastron (CGS)
\newcommand{\hatcurPPfluxperidim}{\ensuremath{8}}                      % flux @ periastron (CGS) units.
\newcommand{\hatcurPPfluxap}{\ensuremath{6.06\pm0.59}}                 % flux @ apastron (CGS)
\newcommand{\hatcurPPfluxapdim}{\ensuremath{8}}                        % flux @ apastron (CGS) units.
\newcommand{\hatcurPPfluxavg}{\ensuremath{7.70_{-1.22}^{+2.42}}}       % flux on average (CGS)
\newcommand{\hatcurPPfluxavgdim}{\ensuremath{8}}                       % flux average (CGS) units.
%% --------------------------------------------------------------------
\newcommand{\hatcurXsecphase}{\ensuremath{0.4589\pm0.0354}}            % Phase of secondary eclipse
\newcommand{\hatcurXsecondary}{\ensuremath{2455242.869\pm0.122}}       % Secondary eclipse epoch
\newcommand{\hatcurXsecdur}{\ensuremath{0.1075\pm0.0109}}              % sec eclipse duration (days)
\newcommand{\hatcurXsecingdur}{\ensuremath{0.0273\pm0.0188}}           % sec I/E duration (days)
\newcommand{\hatcurPPphiconj}{\ensuremath{-0.0654\pm0.1241}}           % phase diff between conjunction and periastron
\newcommand{\hatcurPPperi}{\ensuremath{2455241.51\pm0.43}}             % time of periastron passage.
\newcommand{\hatcurPPaequiv}{\ensuremath{0.0423\pm0.0042}}             % equivalent semi-major axis
\newcommand{\hatcurPPtcirc}{\ensuremath{283.1_{-128.6}^{+169.4}}}      % circularization timescale
\newcommand{\hatcurPPtinfall}{\ensuremath{1151.5_{-460.2}^{+680.8}}}   % infall timescale
%% --------------------------------------------------------------------
\newcommand{\hatcurXdist}{\ensuremath{303_{-23}^{+38}}}                % distance (pc), no reddenning correction
\newcommand{\hatcurXAv}{\ensuremath{0.000\pm0.014}}                    % Av (mag)
\newcommand{\hatcurXdistred}{\ensuremath{297_{-24}^{+38}}}             % distance with Av correction (pc)
\newcommand{\hatcurXEBV}{\ensuremath{0.000\pm0.004}}                   % E(B-V) (mag)
\newcommand{\hatcurXmvisored}{\ensuremath{12.093_{-0.025}^{+0.035}}}   % Expected m_v with reddening (mag)
\newcommand{\hatcurXmiisored}{\ensuremath{11.409\pm0.012}}             % Expected m_i with reddening (mag)
\newcommand{\hatcurXmjisored}{\ensuremath{10.968\pm0.015}}             % Expected m_j with reddening (mag)
\newcommand{\hatcurXmhisored}{\ensuremath{10.628\pm0.028}}             % Expected m_h with reddening (mag)
\newcommand{\hatcurXmkisored}{\ensuremath{10.574_{-0.034}^{+0.025}}}   % Expected m_k with reddening (mag)
\newcommand{\hatcurXviisored}{\ensuremath{0.684_{-0.023}^{+0.031}}}    % Expected V-I with reddening (mag)
\newcommand{\hatcurXvkisored}{\ensuremath{1.518_{-0.045}^{+0.066}}}    % Expected V-K with reddening (mag)
\newcommand{\hatcurXjhisored}{\ensuremath{0.340_{-0.013}^{+0.018}}}    % Expected J-H with reddening (mag)
\newcommand{\hatcurXjkisored}{\ensuremath{0.393_{-0.014}^{+0.021}}}    % Expected J-K with reddening (mag)
\newcommand{\hatcurCCpmra}{\ensuremath{-21.4\pm0.9}}                   % proper motion, in RA
\newcommand{\hatcurCCpmdec}{\ensuremath{-1.2\pm0.9}}                   % proper motion, in DEC
\newcommand{\hatcurCCpm}{\ensuremath{21.4336\pm1.27279}}               % proper motion

